Randomized Manifold Smoothing for Formal Robustness to Semantic Perturbations

Model predictions can be sensitive to small, unrelated variations in the input, which questions the reliability of the model. Randomized smoothing provides robustness guarantees against small, adversarial perturbations, giving a certifiably robust predictor for such perturbations. However, these perturbations are applied across all directions of the ambient space, irrespective of the underlying data manifold. Consequently, its guarantees largely cover perturbations of the input that are not seen in reality rather than semantically meaningful variations in the data. To address this, we introduce \textbf{Randomized Manifold Smoothing}, which adapts the smoothing distribution to local data geometry by shaping Gaussian perturbations along principal directions of a locally estimated subspace. This yields anisotropic certificates over locally supported variations while retaining the statistical certification machinery of randomized smoothing. We evaluate manifold smoothing across image classification, semantic segmentation, interpretable concept representations, and vision-language retrieval tasks, including semantic distribution shifts. Across these settings, we show that manifold smoothing consistently preserves task performance while providing stronger robustness guarantees along semantically meaningful perturbations compared to standard randomized smoothing in high-dimensional data and representation spaces.

==> secs/conc.tex <==
\section{Conclusion}
We introduced Randomized Manifold Smoothing, a framework that provides formal robustness guarantees against perturbations along meaningful data variations. By shaping the smoothing noise with the local covariance of an input's nearest neighbors, our method certifies an ellipsoid aligned with the data manifold rather than an isotropic ball stretching into the ambient space without any relation to the data. This directly addresses the mismatch between adversarial certificates and the variations that actually occur in data. Empirically, we showed that manifold smoothing preserves task performance and certified accuracy at perturbation scales where isotropic smoothing collapses, across classification, segmentation, concept spaces, and vision--language retrieval. Our work shows that certification is not limited to adversarial threat models, but practitioners can obtain guarantees over meaningful input variations, bridging formal robustness and real-world reliability.

==> tables/segmentation_main_metric.tex <==
% \begin{table*}[t]
% \centering

% \caption{
% \textbf{Quantitative segmentation results.}
% We report mIoU, pixel abstention, and the three largest class-wise IoU
% gains of manifold over isotropic smoothing at each noise scale.
% }
% \label{tab:segmentation_quantitative}

% \scriptsize
% \setlength{\tabcolsep}{5pt}
% \renewcommand{\arraystretch}{1.15}

% \begin{tabular}{@{}l c c c c c c@{}}
% \toprule

% $\sigma$
% & 0.02
% & 0.05
% & 0.10
% & 0.30
% & 0.50
% & 1.00
% \\

% \midrule

% $\mathrm{mIoU}_{\mathrm I}\uparrow$
% & 74.03 & 73.10 & 60.76 & 29.87 & 5.39 & 2.12 \\

% $\mathrm{mIoU}_{\mathrm M}\uparrow$
% & \textbf{74.60} & \textbf{74.54} & \textbf{73.37} & \textbf{67.62}
% & \textbf{57.44} & \textbf{35.58} \\

% \addlinespace[2pt]

% $\varnothing_{\mathrm I}\downarrow$
% & 1.88 & 3.60 & \text 3.60 & 23.61 & 40.07 & \textbf{8.81} \\

% $\varnothing_{\mathrm M}\downarrow$
% & \textbf{0.48} & \textbf{1.19} & \textbf{2.45} & \textbf{7.52} & \textbf{13.81} & 30.60 \\

% % \midrule

% % \shortstack[l]{Top-3\\$\Delta$IoU}
% % &
% % \shortstack[l]{
% % R. Ear \upgain{2.56}\\
% % L. Ear \upgain{2.18}\\
% % R. Brow \upgain{1.39}
% % }
% % &
% % \shortstack[l]{
% % R. Eye \upgain{5.8}\\
% % R. Brow \upgain{5.4}\\
% % L. Ear \upgain{5.2}
% % }
% % &
% % \shortstack[l]{
% % L. Eye \upgain{18.2}\\
% % L. Brow \upgain{16.8}\\
% % R. Eye \upgain{15.6}
% % }
% % &
% % \shortstack[l]{
% % L. Eye \upgain{67.7}\\
% % Eye G. \upgain{62.3}\\
% % R. Eye \upgain{60.3}
% % }
% % &
% % \shortstack[l]{
% % Hair \upgain{85.23}\\
% % Nose \upgain{83.19}\\
% % Eye G. \upgain{72.66}
% % }
% % &
% % \shortstack[l]{
% % Skin \upgain{88.60}\\
% % Nose \upgain{84.93}\\
% % Hair \upgain{79.65}
% % }
% % \\

% \bottomrule
% \end{tabular}

% \end{table*}

% FULL WIDTH
% \begin{wraptable}{r}{0.34\textwidth}
% \vspace{-3pt}
% \centering
% \captionsetup{
%     font=scriptsize,
%     labelfont=bf,
%     skip=-3pt
% }

% \caption{
% \textbf{Dense certification on CelebAMask-HQ;}
% Certified mIoU (\%) and pixel abstention rate ($\varnothing$) across noise levels.
% }
% \label{tab:seg_miou}

% \tiny
% \setlength{\tabcolsep}{3.5pt}
% \renewcommand{\arraystretch}{1.05}
% \vspace{4pt}
% \begin{tabular}{@{}c c c c c@{}}
% \toprule

% $\sigma$
% & $\mathrm{mIoU}_{\mathrm I}\uparrow$
% & $\mathrm{mIoU}_{\mathrm M}\uparrow$
% & $\varnothing_{\mathrm I}\downarrow$
% & $\varnothing_{\mathrm M}\downarrow$
% \\

% \midrule

% 0.02
% & 74.03
% & \textbf{74.60}
% & 1.88
% & \textbf{0.48}
% \\

% 0.05
% & 73.10
% & \textbf{74.54}
% & 3.60
% & \textbf{1.19}
% \\

% 0.10
% & 60.76
% & \textbf{73.37}
% & 3.60
% & \textbf{2.45}
% \\

% 0.30
% & 29.87
% & \textbf{67.62}
% & 23.61
% & \textbf{7.52}
% \\

% 0.50
% & 5.39
% & \textbf{57.44}
% & 40.07
% & \textbf{13.81}
% \\

% 1.00
% & 2.12
% & \textbf{35.58}
% & \textbf{8.81}
% & 30.60
% \\

% \bottomrule
% \end{tabular}

% \vspace{-1.5pt}
% \end{wraptable}



% Half left
\begingroup

\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{1.0}

\definecolor{maniBorder}{RGB}{80,170,100}

% ------------------------------------------------------------
% Compact image size
% ------------------------------------------------------------
\newcommand{\segimage}[1]{%
    \includegraphics[width=0.087\textwidth]{#1}%
}

\newcommand{\maniimage}[1]{%
    \begingroup
    \setlength{\fboxsep}{0pt}%
    \setlength{\fboxrule}{0.65pt}%
    \fcolorbox{maniBorder}{white}{%
        \includegraphics[width=0.087\textwidth]{#1}%
    }%
    \endgroup
}

% Reference image + label above
\newcommand{\segcell}[2]{%
    \begin{tikzpicture}[baseline=(img.base)]
        \node[inner sep=0pt,outer sep=0pt] (img) {#1};
        \node[
            overlay,
            font=\tiny,
            anchor=south,
            yshift=-1.7pt
        ] at (img.north) {#2};
    \end{tikzpicture}%
}

% ============================================================
% MAIN LAYOUT
% ============================================================

\begin{tabular}{
    c@{\hspace{2.5pt}}
    c@{\hspace{2.5pt}}
    c@{\hspace{1.5pt}}
    c@{\hspace{1.5pt}}
    c@{\hspace{1.5pt}}
    c@{\hspace{1.5pt}}
    c
}

% ------------------------------------------------------------
% Increasing noise
% ------------------------------------------------------------
&
&
\multicolumn{5}{c}{
    \begin{tikzpicture}[baseline]
        \node[font=\tiny] (n) {Increasing noise $\sigma$};
        \draw[->,thin,gray!65]
        ([xshift=-1.45cm,yshift=-0.1mm]n.south)
        --
        ([xshift=1.45cm,yshift=-0.1mm]n.south);
    \end{tikzpicture}
}
\\[-4pt]

% ------------------------------------------------------------
% Sigma labels
% ------------------------------------------------------------
&
&
{\tiny $0.02$}
&
{\tiny $0.10$}
&
{\tiny $0.30$}
&
{\tiny $0.50$}
&
{\tiny $1.00$}
\\[-1pt]

% ============================================================
% ISOTROPIC
% ============================================================

\segcell{
    \segimage{
        figures/experiment/segmentation/segmentation_samples/sample_0000_0.1_noise/original.png
    }
}{Sample $x$}
&
\raisebox{1.35\height}{%
    \rotatebox[origin=c]{90}{\tiny Isotropic}%
}
&
\segimage{
    figures/experiment/segmentation/segmentation_samples/sample_0000_0.02_noise/isotropic_certified_mask.png
}
&
% --- annotated sigma=0.10 ---
\begin{tikzpicture}[baseline=(iso010.base)]
    \node[inner sep=0pt,outer sep=0pt] (iso010) {
        \includegraphics[width=0.087\textwidth]{
            figures/experiment/segmentation/segmentation_samples/sample_0000_0.1_noise/isotropic_certified_mask.png
        }
    };

    \node[
        font=\fontsize{3.6}{4}\selectfont,
        text=white,
        anchor=west,
        fill=black,
        fill opacity=0.55,
        text opacity=1,
        inner sep=0.5pt
    ] (browlabel)
    at ([xshift=-6.7mm,yshift=-1.4mm]iso010.north east)
    {R. Eye};

    \draw[
        ->,
        line width=0.3pt,
        white
    ]
    (browlabel.south east)
    --
    ([xshift=2.8mm,yshift=1.5mm]iso010.center);
\end{tikzpicture}
&
\segimage{
    figures/experiment/segmentation/segmentation_samples/sample_0000_0.3_noise/isotropic_certified_mask.png
}
&
\segimage{
    figures/experiment/segmentation/segmentation_samples/sample_0000_0.5_noise/isotropic_certified_mask.png
}
&
\segimage{
    figures/experiment/segmentation/segmentation_samples/sample_0000_1.00_noise/isotropic_certified_mask.png
}
\\[1.5pt]

% ============================================================
% MANIFOLD
% ============================================================

\segcell{
    \segimage{
        figures/experiment/segmentation/segmentation_samples/sample_0000_0.1_noise/gt_mask.png
    }
}{GT-Mask}
&
\raisebox{0.80\height}{%
    \rotatebox[origin=c]{90}{\tiny\textbf{Manifold} (Ours)}%
}
&
\maniimage{
    figures/experiment/segmentation/segmentation_samples/sample_0000_0.02_noise/manifold_certified_mask.png
}
&
\maniimage{
    figures/experiment/segmentation/segmentation_samples/sample_0000_0.1_noise/manifold_certified_mask.png
}
&
\maniimage{
    figures/experiment/segmentation/segmentation_samples/sample_0000_0.3_noise/manifold_certified_mask.png
}
&
\maniimage{
    figures/experiment/segmentation/segmentation_samples/sample_0000_0.5_noise/manifold_certified_mask.png
}
&
\maniimage{
    figures/experiment/segmentation/segmentation_samples/sample_0000_1.00_noise/manifold_certified_mask.png
}

\end{tabular}

\endgroup
